CLiMB: A Continual Learning Benchmark for Vision-and-Language Tasks

Current state-of-the-art vision-and-language models are evaluated on tasks either individually or in a multi-task setting, overlooking the challenges of continually learning (CL) tasks as they arrive. Existing CL benchmarks have facilitated research on task adaptation and mitigating "catastrophic forgetting", but are limited to vision-only and language-only tasks. We present CLiMB, a benchmark to study the challenge of learning multimodal tasks in a CL setting, and to systematically evaluate how upstream continual learning can rapidly generalize to new multimodal and unimodal tasks. CLiMB includes implementations of several CL algorithms and a modified Vision-Language Transformer (ViLT) model that can be deployed on both multimodal and unimodal tasks. We find that common CL methods can help mitigate forgetting during multimodal task learning, but do not enable cross-task knowledge transfer. We envision that CLiMB will facilitate research on a new class of CL algorithms for this challenging multimodal setting.

==> tasks_table.tex <==

\begin{table}[t]
  \small
  \centering
  \begin{tabular}{llll}
    \toprule
    \bf Name & \bf Task & \bf Vision Input(s) & \bf Language Input(s) \\% & \bf Source \\
    \midrule
    VQAv2 & Visual QA  & 1 image & 1 question \\%& COCO \\
    NLVR2 & Visual Reasoning & 2 images & 1 text description \\%& Google Images \\
    SNLI-VE & Visual Entailment & 1 image & 1 text hypothesis \\%& SNLI; Flickr30K \\
    VCR  & Visual Reasoning & \makecell[l]{1 image w/ \\ object boxes} & \makecell[l]{1 grounded question, \\ 4 grounded options} \\%& LSMDC; MovieClips \\
    \midrule
    SST-2  & Sentiment Cls. & N/A & 1 sentence \\%& rottentomatoes.com \\
    IMDb  & Sentiment Cls. & N/A & 1 sentence \\%& imdb.com \\
    HellaSwag  & Sentence continuation & N/A & 1 context, 4 options \\%& \\%\makecell[l]{ActivityNet Captions; \\ WikiHow} \\
    %Cosmos QA  & commonsense reasoning & N/A & 1 context; 1 question; 4 options &  Spinn3r Blog \\
    CommonsenseQA & commonsense QA & N/A & 1 question, 5 options \\%& ConceptNet \\
    PIQA & physical reasoning & N/A & 1 context, 2 options \\%& instructables.com \\
    \midrule
    ImageNet-1000 & image classification & 1 image & N/A \\%& ILSVRC2012 \\
    iNaturalist2019 & image classification & 1 image & N/A \\
    Places365 & image classification & 1 image & N/A \\
    COCO-obj det & multi-label image classification & 1 image & N/A \\
    \bottomrule
  \end{tabular}
  \caption{Overview of the tasks in the proposed continual learning benchmark.}
  \label{tab:old_benchmark}
\end{table}
